S3A: Secure System Simplex Architecture for Enhanced Security of Cyber-Physical Systems

Until recently, cyber-physical systems, especially those with safety-critical properties that manage critical infrastructure (e.g. power generation plants, water treatment facilities, etc.) were considered to be invulnerable against software security breaches. The recently discovered 'W32.Stuxnet' worm has drastically changed this perception by demonstrating that such systems are susceptible to external attacks. Here we present an architecture that enhances the security of safety-critical cyber-physical systems despite the presence of such malware. Our architecture uses the property that control systems have deterministic execution behavior, to detect an intrusion within 0.6 {\mu}s while still guaranteeing the safety of the plant. We also show that even if an attack is successful, the overall state of the physical system will still remain safe. Even if the operating system's administrative privileges have been compromised, our architecture will still be able to protect the physical system from coming to harm.

==> pred_sched.tex <==
\subsection{Predictable Scheduling}

% This subsection describes an OS scheduler-based technique that
% considerably improves the determinism of the system and enhances the ability 
% to detect intrusion more easily.

%The technique described in Section \ref{subsec:time} can be compromised if,
%for example, an attacker has the source code of the control software and is
%able to replace it with a modified one. As we already explained this
%is very hard to realize since in most cases S3A will detect the attempt to
%substitute the controller. However, assuming that the attacker finds a way to
%do so, she could potentially replicate the side channel, as long as the new
%(malicious) controller sends the same timing signals at the same time and same
%frequency.

%However, even when an attacker has modified the control software so that it
%bypasses the timing and instruction-based detection mechanisms, the total
%scheduling behavior observed by the operating system will be different. {\em
%E.g.}, if malicious code is added before or after the timing/instruction
%counts have been communicated with the FPGA, the total execution time of the
%system would be still different, thus resulting in different scheduling
%behavior. % invoke a new process?

%Therefore, adding an operating system scheduler hook that collects time and
%instruction count at each scheduling event and sending them to the FPGA can further
%improve the security because deviations from normal scheduling behavior could be
%an indication of malicious code infection, of course assuming normal scheduling
%behavior is regular. Fortunately, the scheduling behavior of control systems is
%typically regular with very small variability.

A {\em deterministic real-time scheduler} \cite{Yun:DRTS-RTASWIP} 
improves determinism by utilizing the instruction count of the control code. 
The scheduler uses the instruction counts for scheduling decisions {\em i.e.},
context switching after executing a certain number of instructions. 
Time is also monitored at every scheduling point so that it does not 
violate real-time constraints. Hence, the system schedule can be completely
deterministic with an instruction-level granularity w.r.t. a given set of
inputs. Employing this technique ensures that any deviation from the 
known schedule, even of a single instruction, can be treated as an
indication of the existence of malicious code. 

To compromise this deterministic scheduling event based technique, an
attacker should {\em (1)} know the complete scheduling behavior of the system
with instruction-level granularity and {\em (2)} replace the part of OS that
collects and sends the information about the scheduling events. Both of these
are extremely hard to do and therefore significantly increases the level of
difficulty for the would-be attackers.


